Wireless Picosecond Time Synchronization for Distributed Antenna Arrays

Distributed antenna arrays have been proposed for many applications ranging from space-based observatories to automated vehicles. Achieving good performance in distributed antenna systems requires stringent synchronization at the wavelength and information level to ensure that the transmitted signals arrive coherently at the target, or that scattered and received signals can be appropriately processed via distributed algorithms. In this paper we address the challenge of high precision time synchronization to align the operations of elements in a distributed antenna array and to overcome time-varying bias between platforms due to oscillator drift. We use a spectrally sparse two-tone waveform, which obtains approximately optimal time estimation accuracy, in a two-way time transfer process. We also describe a technique for determining the true time delay using the ambiguous two-tone matched filter output, and we compare the time synchronization precision of the two-tone waveform with the more common linear frequency modulation (LFM) waveform. We experimentally demonstrate wireless time synchronization using a single pulse 40$\,$MHz two-tone waveform over a 90$\,$cm 5.8$\,$GHz wireless link in a laboratory setting, obtaining a timing precision of 2.26$\,$ps.

==> arxiv_submission_v2.0/acronyms.tex <==
% --- Acronyms ------------------------

% Signals/Signal Processing
\DeclareAcronym{ls}{
	short = LS,
	long = least-squares
}
\DeclareAcronym{qls}{
	short = QLS,
	long = quadratic least-squares
}
\DeclareAcronym{sinc-ls}{
	short = sinc-LS,
	long = sinc nonlinear least-squares
}
\DeclareAcronym{mf-ls}{
	short = MFLS,
	long = matched filter least-squares
}
\DeclareAcronym{rf}{
	short = RF,
	long = radio frequency
}
\DeclareAcronym{lfm}{
	short = LFM,
	long = linear frequency modulation
}
\DeclareAcronym{prf}{
	short = PRF,
	long = pulse repetition frequency
}
\DeclareAcronym{pri}{
	short = PRI,
	long = pulse repetition interval
}
\DeclareAcronym{fmcw}{
	short = FMCW,
	long = frequency modulated continuous-wave
}
\DeclareAcronym{lfmcw}{
	short = LFMCW,
	long = linear frequency modulated continuous-wave
}
\DeclareAcronym{cw}{
	short = CW,
	long = continuous-wave
}
\DeclareAcronym{dbf}{
	short = DBF,
	long = digital beamforming
}
\DeclareAcronym{sar}{
	short = SAR,
	long = synthetic aperture radar
}
\DeclareAcronym{psr}{
	short = PSR,
	long = point scatterer response
}
\DeclareAcronym{rcs}{
	short = RCS,
	long = radar cross-section
}
\DeclareAcronym{crlb}{
	short = CRLB,
	long = Cramer-Rao lower bound
}
\DeclareAcronym{dof}{
	short = DoF,
	long = degree of freedom
}
\DeclareAcronym{snr}{
	short = SNR,
	long = signal-to-noise ratio
}
\DeclareAcronym{sinr}{
	short = SINR,
	long = signal-to-interference-plus-noise ratio
}
\DeclareAcronym{fft}{
	short = FFT,
	long = fast Fourier transform,
}
\DeclareAcronym{ifft}{
	short = IFFT,
	long = inverse \ac{fft},
}
\DeclareAcronym{ift}{
	short = IFT,
	long = inverse Fourier transform,
}
\DeclareAcronym{rms}{
	short = RMS,
	long = root-mean-square
}
\DeclareAcronym{rmse}{
	short = RMSE,
	long = \ac{rms} error
}
\DeclareAcronym{psd}{
	short = PSD,
	long = power spectral density
}
\DeclareAcronym{rca}{
	short = RCA,
	long = range of closest approach
}
\DeclareAcronym{rda}{
	short = RDA,
	long = Range-Doppler Algorithm
}
\DeclareAcronym{rma}{
	short = RMA,
	long = Range Migration Algorithm
}
\DeclareAcronym{pfa}{
	short = PFA,
	long = Polar Formatting Algorithm
}
\DeclareAcronym{bpa}{
	short = BPA,
	long = Backprojection Algorithm
}
\DeclareAcronym{rvp}{
	short = RVP,
	long = residual video phase
}
\DeclareAcronym{jrc}{
	short = JRC,
	long = joint radar-communications
}
\DeclareAcronym{doa}{
	short = DOA,
	long = direction of arrival
}
\DeclareAcronym{hci}{
	short = HCI,
	long = human-computer interaction
}
\DeclareAcronym{its}{
	short = ITS,
	long = intelligent transportation systems
}
\DeclareAcronym{rtk}{
	short = RTK,
	long = real-time kinematic
}
\DeclareAcronym{eirp}{
	short = EIRP,
	long = effective isotropic radiated power
}
\DeclareAcronym{gnss}{
	short = GNSS,
	long = global navigation satellite system
}
\DeclareAcronym{imu}{
	short = IMU,
	long = inertial measurement unit
}


% Communications
\DeclareAcronym{ofdm}{
	short = OFDM,
	long = orthogonal frequency division multiplexing
}
\DeclareAcronym{los}{
	short = LoS,
	long = line of sight
}


% Hardware
\DeclareAcronym{pll}{
	short = PLL,
	long = phase-locked loop
}
\DeclareAcronym{vco}{
	short = VCO,
	long = voltage-controlled oscillator
}
\DeclareAcronym{lna}{
	short = LNA,
	long = low-noise amplifier
}
\DeclareAcronym{if}{
	short = IF,
	long = intermediate frequency
}
\DeclareAcronym{cots}{
	short = COTS,
	long = commercial off-the-shelf
}
\DeclareAcronym{adc}{
	short = ADC,
	long = analog to digital converter
}
\DeclareAcronym{dac}{
	short = DAC,
	long = digital to analog converter
}
\DeclareAcronym{lo}{
	short = LO,
	long = local oscillator
}
\DeclareAcronym{pcb}{
	short = PCB,
	long = printed circuit board
}
\DeclareAcronym{mimo}{
	short = MIMO,
	long = multiple-input multiple-output
}
\DeclareAcronym{simo}{
	short = SIMO,
	long = single-input multiple-output
}
\DeclareAcronym{mmic}{
	short = MMIC,
	long = monolithic microwave integrated circuit
}
\DeclareAcronym{daq}{
	short = DAQ,
	long = data acquisition
}
\DeclareAcronym{ic}{
	short = IC,
	long = integrated circuit
}
\DeclareAcronym{pa}{
	short = PA,
	long = power amplifier
}



% Company acronyms
\DeclareAcronym{ti}{
	short = TI,
	long = Texas Instruments
}
\DeclareAcronym{adi}{
	short = ADI,
	long = Analog Devices
}


% Misc.
\DeclareAcronym{roi}{
	short = ROI,
	long = region of interest,
	long-plural-form = regions of interest
}
\DeclareAcronym{v2x}{
	short = V2X,
	long = vehicle-to-everything
}
\DeclareAcronym{av}{
	short = AV,
	long = automated vehicle
}
\DeclareAcronym{cors}{
	short = CORS,
	long = continuously operating reference station
}
\DeclareAcronym{mdot}{
	short = MDOT,
	long = Michigan Department of Transportation
}
\DeclareAcronym{moco}{
	short = MOCO,
	long = motion compensation
}
\DeclareAcronym{sdr}{
	short = SDR,
	long = software-defined radio
}
\DeclareAcronym{gpio}{
	short = GPIO,
	long = general-purpose input/output
}
\DeclareAcronym{usrp}{
	short = USRP,
	long = Universal Software Radio Peripheral
}
\DeclareAcronym{uhd}{
	short = UHD,
	long = \ac{usrp} Hardware Driver
}
\DeclareAcronym{ntp}{
	short = NTP,
	long = network time protocol
}
\DeclareAcronym{ptp}{
	short = PTP,
	long = precision time protocol
}
\DeclareAcronym{lan}{
	short = LAN,
	long = local area network
}
\DeclareAcronym{wlan}{
	short = WLAN,
	long = wireless \ac{lan}
}
\DeclareAcronym{lut}{
	short = LUT,
	long = lookup table
}
\DeclareAcronym{wsn}{
	short = WSN,
	long = wireless sensor network
}
\DeclareAcronym{mac}{
	short = MAC,
	long = media access control
}
\DeclareAcronym{pps}{
	short = PPS,
	long = pulse-per-second
}
\DeclareAcronym{fom}{
	short = FoM,
	long = figure of merit
}
\DeclareAcronym{uwb}{
	short = UWB,
	long = ultra-wideband
}

